Fusion of Head and Full-Body Detectors for Multi-Object Tracking

In order to track all persons in a scene, the tracking-by-detection paradigm has proven to be a very effective approach. Yet, relying solely on a single detector is also a major limitation, as useful image information might be ignored. Consequently, this work demonstrates how to fuse two detectors into a tracking system. To obtain the trajectories, we propose to formulate tracking as a weighted graph labeling problem, resulting in a binary quadratic program. As such problems are NP-hard, the solution can only be approximated. Based on the Frank-Wolfe algorithm, we present a new solver that is crucial to handle such difficult problems. Evaluation on pedestrian tracking is provided for multiple scenarios, showing superior results over single detector tracking and standard QP-solvers. Finally, our tracker ranks 2nd on the MOT16 benchmark and 1st on the new MOT17 benchmark, outperforming over 90 trackers.

==> results/experiment/GT.tex <==
%\captionsetup[subtable]{labelformat=simple,labelsep=colon}
\begin{table}[htp]
	\begin{center}
			\label{tab:FW_solver_comparison}
		\tabcolsep=0.05cm
    \renewcommand{\arraystretch}{0.55}
   			\caption{Solver comparisons (body+head detections) on the entire MOT16train set.} \bigskip
			\begin{tabular}{lcccc}
				\toprule
				{Solver} & {IDF1} & {ID} & {FM} & {MOTA}\\
				\midrule
				{FW} & 16.7 & 1207 & 724 & 31.1\\
				{FW+\regulizer} & 26.8 & 807 & 802 & 33.4\\
				{FW+\regulizer+h} & 42.9 & 372 & 724 & 38.2\\
				\bottomrule
			\end{tabular}
				\end{center}
\end{table}


==> results/mot16/CEM.tex <==
CEM \cite{Milan:2014:PAMI} & 33.2$\pm$7.9	& 75.8	& 1.2& 	7.8& 	54.4& 	6837& 	114322& 	642 (17.2)	& 731 (19.6)
\\


==> results/mot16/DP_NMS.tex <==
DP\_NMS \cite{Pirsiavash:2011:CVPR} & 32.2$\pm$9.8&	76.4	&0.2	&5.4&	62.1&	1123&	121579&	972 (29.2)&	944 (28.3)
\\


==> results/mot16/EAMTT_pub.tex <==
EAMTT\_pub \cite{sanchezbmtt2016} & 38.8$\pm$8.5&75.1&	1.4	&7.9&	49.1&	8114&	102452	&965 (22.0)	&1657 (37.8)
\\


==> results/mot16/GMPHD_HDA.tex <==
GMPHD\_HDA \cite{SongICCE2016} & 30.5$\pm$6.9&	75.4&	0.9	&4.6&	59.7&	5169	&120970	&539 (16.0)&	731 (21.7)
\\


==> results/mot16/JMC.tex <==
JMC \cite{tangBMTT2016} & 46.3$\pm$9.0	& 75.7& 	1.1	& 15.5& 	39.7& 	6373	& 90914& 	657 (13.1)	& 1114 (22.2)\\


==> results/mot16/JPDA_m.tex <==
JPDA\_m \cite{Rezatofighi:2015:ICCV} & 26.2$\pm$6.1&	76.3	&0.6	&4.1&	67.5&	3689	&130549	&365 (12.9)&	638 (22.5)
\\


==> results/mot16/LINF1.tex <==
LINF1 \cite{FagotECCV2016} & 41.0$\pm$9.5&	74.8	&1.3&	11.6&	51.3&	7896	&99224&	430 (9.4)	&963 (21.1)
\\


==> results/mot16/LP2D.tex <==
LP2D \cite{lealiccv2011} & 35.7$\pm$10.1&	75.8&	0.9&	8.7&	50.7&	5084	&111163&	915 (23.4)&	1264 (32.4)\\


==> results/mot16/LTTSC-CRF.tex <==
LTTSC-CRF \cite{LeBMTT2016} & 37.6$\pm$0.0	&75.9	&2	&9.6&	55.2&	11969&	101343	&481 (10.8)&	1012 (22.8)
\\

==> results/mot16/MDPNN16.tex <==
MDPNN16 \cite{SadeghianArxiv2017} & 43.8$\pm$7.3	& 75.5	& 0.6	& 12.4& 	40.7& 	3501& 	98193& 	723 (15.7)	& 2036 (44.1)\\



==> results/mot16/MHT_DAM.tex <==
MHT\_DAM \cite{Kim:2015:ICCV} & 42.9$\pm$8.9&	76.6&	1&	13.6&	46.9&	5668&	97919	&499 (10.8)&	659 (14.2)
 \\


==> results/mot16/NLLMPa.tex <==
NLLMPa \cite{levinkovcvpr2017} & 47.6$\pm$10.6&	78.5	& 1.0	&17.0&	40.4&	5844&	89093&	629 (12.3)&	768 (15.0)
\\


==> results/mot16/NOMT.tex <==
NOMT \cite{Choi:2015:ICCV} & 46.4$\pm$9.9	&76.6&	1.6&	18.3&	41.4&	9753&	87565&	359 (6.9)&	504 (9.7)\\



==> results/mot16/OVBT.tex <==
OVBT \cite{BanBMTT2016} & 38.4$\pm$8.8&	75.4 &	1.9	 &7.5 &	47.3 &	11517 &	99463 &	1321 (29.1)	 &2140 (47.1)
\\

==> results/mot16/SMOT.tex <==
SMOT \cite{Dicle:2013:ICCV} & 29.7$\pm$7.3&	75.2	&2.9	&5.3&	47.7&	17426&	107552&	3108 (75.8)&	4483 (109.3)
 \\


==> results/mot16/TBD.tex <==
TBD \cite {Geiger:2014:PAMI} & 33.7$\pm$9.2	&76.5&	1&	7.2&	54.2&	5804&	112587	&2418 (63.2)	&2252 (58.9)
\\


==> results/mot16/olCF.tex <==
olCF \cite{kieritzAVSS2016} & 43.2$\pm$10.2	& 74.3	& 1.1	& 11.3& 48.5& 	6651& 	96515	& 381 (8.1)& 	1404 (29.8)
 \\


==> results/mot16_onecol/AMIR.tex <==
AMIR \cite{Sadeghian:ICCV:2017} & 4 & 47.2&	46.3&	14.0&	41.6&	2681&	92856	&774 &	1675 
 \\


==> results/mot16_onecol/CEM.tex <==
CEM \cite{milantpami2014} & 33.2	& 75.8	&	7.8& 	54.4& 	6837& 	114322& 	642 	& 731 
\\


==> results/mot16_onecol/DP_NMS.tex <==
DP\_NMS \cite{Pirsiavash:2011:CVPR} & 65 & 26.6 &	31.2	& 4.1&	67.5&	3689&	130557&	365&	638 
\\


==> results/mot16_onecol/EAMTT_pub.tex <==
EAMTT\_pub \cite{sanchezbmtt2016} & 38.8&75.1&	7.9&	49.1&	8114&	102452	&965 	&1657 
\\

==> results/mot16_onecol/GMPHD_HDA.tex <==
GMPHD\_HDA \cite{SongICCE2016} & 30.5&	75.4&	4.6&	59.7&	5169	&120970	&539 &	731
\\


==> results/mot16_onecol/JMC.tex <==
JMC \cite{tangBMTT2016} & 46.3	& 75.7& 	15.5& 	39.7& 	6373	& 90914 & 	657	& 1114\\


==> results/mot16_onecol/JPDA_m.tex <==
JPDA\_m \cite{Rezatofighi:2015:ICCV} & 26.2&	76.3		&4.1&	67.5&	3689	&130549	&365 &	638 
\\


==> results/mot16_onecol/LINF1.tex <==
LINF1 \cite{FagotECCV2016} & 41.0&	74.8&	11.6&	51.3&	7896	&99224&	430	&963
\\


==> results/mot16_onecol/LMP.tex <==
LMP \cite{liftedTrack2017} & 1 &{\bf 48.8}	& {\bf 51.3}& 	18.2& 	40.1& 	6654	& 86245 & 	{\bf 481}	& {\bf 595}\\


==> results/mot16_onecol/LP2D.tex <==
LP2D \cite{lealiccv2011} & 35.7&	75.8&	8.7&	50.7&	5084	&111163&	915 &	1264 \\


==> results/mot16_onecol/LTTSC-CRF.tex <==
LTTSC-CRF \cite{LeBMTT2016} & 37.6&75.9	&9.6&	55.2&	11969&	101343	&481 &	1012 
\\

==> results/mot16_onecol/MDPNN16.tex <==
MDPNN16 \cite{SadeghianArxiv2017} & 43.8	& 75.5 & 12.4& 	40.7& 	3501& 	98193& 	723 & 2036 \\



==> results/mot16_onecol/MHT_DAM.tex <==
MHT\_DAM \cite{Kim:2015:ICCV} & 42.9&	{\bf 76.6}&	13.6&	46.9&	5668&	97919	&499 &	659 
 \\


==> results/mot16_onecol/NLLMPa.tex <==
NLLMPa \cite{levinkov2017joint} & 3 &47.6	& 47.3& 	17.0& 	40.4& 	{\bf 5844}	& 89093 & 	629	& 768\\


==> results/mot16_onecol/NOMT.tex <==
NOMT \cite{choiiccv2015} & 5 & 46.4	&{\bf 53.3}&	18.3&	41.4&	9753&	87565&	{\bf 359} &	{\bf 504}\\



==> results/mot16_onecol/OVBT.tex <==
OVBT \cite{BanBMTT2016} & 38.4&	75.4  &7.5 &	47.3 &	11517 &	99463 &	1321	 &2140 \\

==> results/mot16_onecol/SMOT.tex <==
SMOT \cite{Dicle:2013:ICCV} & 29.7&	75.2		&5.3&	47.7&	17426&	107552&	3108&	4483
 \\


==> results/mot16_onecol/TBD.tex <==
TBD \cite {Geiger:2014:PAMI} & 33.7	&76.5&		7.2&	54.2&	5804&	112587	&2418	&2252
\\


==> results/mot16_onecol/olCF.tex <==
oICF \cite{kieritzAVSS2016} & 43.2	& 74.3		& 11.3& 48.5& 	6651& 	96515	& 381 & 	1404
 \\

